Anomaly detection in the dynamics of web and social networks

In this work, we propose a new, fast and scalable method for anomaly detection in large time-evolving graphs. It may be a static graph with dynamic node attributes (e.g. time-series), or a graph evolving in time, such as a temporal network. We define an anomaly as a localized increase in temporal activity in a cluster of nodes. The algorithm is unsupervised. It is able to detect and track anomalous activity in a dynamic network despite the noise from multiple interfering sources. We use the Hopfield network model of memory to combine the graph and time information. We show that anomalies can be spotted with a good precision using a memory network. The presented approach is scalable and we provide a distributed implementation of the algorithm. To demonstrate its efficiency, we apply it to two datasets: Enron Email dataset and Wikipedia page views. We show that the anomalous spikes are triggered by the real-world events that impact the network dynamics. Besides, the structure of the clusters and the analysis of the time evolution associated with the detected events reveals interesting facts on how humans interact, exchange and search for information, opening the door to new quantitative studies on collective and social behavior on large and dynamic datasets.

==> visualization.tex <==
\section{Graph visualization and community detection}\label{visualization}

The structure of each learned network shows patterns corresponding to communities of correlated nodes. We analyze all the monthly Hopfield networks, extract communities and visualize them in the following sections.
We use a heuristic method based on modularity optimization (Louvain method) \cite{blondel2008fast} for community detection. Colors in the graph depict and highlight the detected communities. A resolution parameter controls the size of communities.
To represent the graph in 2D space for visualization, we use a force-directed layout \cite{jacomy2014forceatlas2}. The resulting spatial layout reflects the organization of the network. An interactive version of all visualizations presented in this paper is available online \cite{WikiViz}.

%weight distribution
\begin{figure}[t!]
	\centering
	%    \captionsetup{justification=centering}
	\includegraphics[width=\columnwidth]{figures/edge_weight_distribution.pdf}
	\caption{Edge weight distribution in the learned graph in log scale. The learned graph has skewed heavy-tailed weight distribution.}
	\label{fig: edge_weight_distribution}
\end{figure}

